Dual-Solver: A Generalized ODE Solver for Diffusion Models with Dual Prediction

Diffusion models achieve state-of-the-art image quality. However, sampling is costly at inference time because it requires a large number of function evaluations (NFEs). To reduce NFEs, classical ODE numerical methods have been adopted. Yet, the choice of prediction type and integration domain leads to different sampling behaviors. To address these issues, we introduce Dual-Solver, which generalizes multistep samplers through learnable parameters that continuously (i) interpolate among prediction types, (ii) select the integration domain, and (iii) adjust the residual terms. It retains the standard predictor-corrector structure while preserving second-order local accuracy. These parameters are learned via a classification-based objective using a frozen pretrained classifier (e.g., MobileNet or CLIP). For ImageNet class-conditional generation (DiT, GM-DiT) and text-to-image generation (SANA, PixArt-$\alpha$), Dual-Solver improves FID and CLIP scores in the low-NFE regime ($3 \le$ NFE $\le 9$) across backbones.

==> experiment/training_time/main.tex <==
\subsection{Training Time}
\label{sec:training_time}
% Requires: \usepackage{caption}
\noindent
\begin{minipage}[h]{0.46\textwidth}
\centering
  \includegraphics[width=\linewidth]{experiment/training_time/figs/time.png}
  \captionsetup{aboveskip=2pt,belowskip=0pt}
  \captionof{figure}{Training time per step (ms) (Table~\ref{tab:training_time_per_step}).}
  \label{fig:training_time}
\end{minipage}\hfill%  <-- 공백 제거용 %
\begin{minipage}[h]{0.53\textwidth}
Fig.~\ref{fig:training_time} reports per-step training time, decomposed into sampling, decoding, classifier, and backward, measured at NFE $=5$ using GM-DiT~\citep{chen2025gaussian} as the backbone. Dual-Solver adds decoding and classifier overheads; the latter is modest thanks to lightweight choices, as discussed in Sec.~\ref{para:classifier_model_selection} (D). Overall, total per-step time increases by about $8\%$ versus BNS-Solver~\citep{shaul2024bespoke} and DS-Solver~\citep{wang2025differentiable}. See Appendix~\ref{app:analysis_of_training_time} for convergence-time details.
\end{minipage}

